Learning-Aided Control of Robotic Tether-Net with Maneuverable Nodes to Capture Large Space Debris

Maneuverable tether-net systems launched from an unmanned spacecraft offer a promising solution for the active removal of large space debris. Guaranteeing the successful capture of such space debris is dependent on the ability to reliably maneuver the tether-net system -- a flexible, many-DoF (thus complex) system -- for a wide range of launch scenarios. Here, scenarios are defined by the relative location of the debris with respect to the chaser spacecraft. This paper represents and solves this problem as a hierarchically decentralized implementation of robotic trajectory planning and control and demonstrates the effectiveness of the approach when applied to two different tether-net systems, with 4 and 8 maneuverable units (MUs), respectively. Reinforcement learning (policy gradient) is used to design the centralized trajectory planner that, based on the relative location of the target debris at the launch of the net, computes the final aiming positions of each MU, from which their trajectory can be derived. Each MU then seeks to follow its assigned trajectory by using a decentralized PID controller that outputs the MU's thrust vector and is informed by noisy sensor feedback (for realism) of its relative location. System performance is assessed in terms of capture success and overall fuel consumption by the MUs. Reward shaping and surrogate models are used to respectively guide and speed up the RL process. Simulation-based experiments show that this approach allows the successful capture of debris at fuel costs that are notably lower than nominal baselines, including in scenarios where the debris is significantly off-centered compared to the approaching chaser spacecraft.

==> tables/symsParam.tex <==
\caption{\label{tab:table1} Simulation Parameters.}
\centering
\begin{tabular}{lcccc}
\hline
Parameter&Value\\\hline
\multicolumn{5}{c}{\textbf{Chaser, Tether, and Winch}}\\
\hline
Chaser Side Length $L_{ch}$, m & 1.5\\
Chaser Mass $m_{ch}$, kg & 1600\\
Chaser and Net Initial Distance $d_{ch}$, m & 0.1\\
Winch Radius $r_{w}$, m & 0.05\\
Winch Height $h_{w}$, m & 0.02\\
Winch Mass $m_{w}$, kg& 0.1\\
Tether Radius $r_{t}$, m & 0.002\\
Tether Density $\rho_{t}$, kg/m$^3$& 1390\\
Tether Young's Modulus $E_{t}$, GPA& 70\\
Tether Axial Damping Ratio $c_{t}$& 0.106\\
\hline
\label{tab:nominalparams}\\
\end{tabular}
\quad
\begin{tabular}{lcccc}
\hline
Parameter&Value\\\hline
\multicolumn{5}{c}{\textbf{Net, Corner Threads, and MU}}\\
\hline
Side Length $L_{net}$, m& 22.0\\
Mesh Length $l_{net,0}$, m& 1.0\\
Thread Radius $r_{net}$, m& 0.0011\\
Thread Density $\rho_{net}$, kg/m$^3$& 1390.0\\
Net Young's Modulus $E_{net}$, GPA& 70\\
Net Axial Damping Ratio $c_{net}$& 0.106\\
Corner Thread Length $l_{CT,0}$, m& 1.4142\\
Corner Thread Radius $r_{CT}$, m& 0.0007 \\
MU radius, $r_{MU}$, m& 0.0605 \\
\hline
\label{tab:nominalparams}\\
\end{tabular}
\begin{tabular}{lcccc}
\hline
Parameter&Value\\
\hline
\multicolumn{5}{c}{\textbf{Initial Conditions and Timestep}}\\
\hline
MU Ejection Speed $v_{e}$, m/s& 2.5\\
MU Shooting Angle $\theta_e$, deg &     36.87 \\
Net Stowed Side Length $L_{net,0}$, m  &     1.1 & \\
Simulation Time Step $\Delta$t, s & 10$^{-2}$\\
\hline
\end{tabular}


==> tables/symsParam_2.tex <==
\caption{\label{tab:table1} Simulation Parameters.}
\centering
% \begin{adjustbox}{width=1\textwidth}
\begin{tabular}{lcccc}
\hline
Parameter&Value\\\hline
\multicolumn{5}{c}{\textbf{Chaser, Tether, and Winch}}\\
\hline
Chaser Side Length $L_{ch}$, m & 1.5\\
Chaser Mass $m_{ch}$, kg & 1600\\
Chaser and Net Initial Distance $d_{ch}$, m & 0.1\\
Winch Radius $r_{w}$, m & 0.05\\
Winch Height $h_{w}$, m & 0.02\\
Winch Mass $m_{w}$, kg& 0.1\\
Tether Radius $r_{t}$, m & 0.002\\
Tether Density $\rho_{t}$, kg/m$^3$& 1390\\
Tether Young's Modulus $E_{t}$, GPA& 70\\
Tether Axial Damping Ratio $c_{t}$& 0.106\\
\hline
\multicolumn{5}{c}{\textbf{Net and Corner Threads}}\\
\hline
Side Length $L_{net}$, m& 22.0\\
Mesh Length $l_{net,0}$, m& 1.0\\
Thread Radius $r_{net}$, m& 0.0011\\
Thread Density $\rho_{net}$, kg/m$^3$& 1390.0\\
Net Young's Modulus $E_{net}$, GPA& 70\\
Net Axial Damping Ratio $c_{net}$& 0.106\\
Corner Thread Length $l_{CT,0}$, m& 1.4142\\
Corner Thread Radius $r_{CT}$, m& 0.0007 \\
\hline
\multicolumn{5}{c}{\textbf{Initial Conditions}}\\
\hline
MU Ejection Speed $v_{e}$, m/s& 2.5\\
MU Shooting Angle $\theta_e$, deg &     36.87 \\
Net Stowed Side Length $L_{net,0}$, m  &     1.1 & \\
\hline
\multicolumn{5}{c}{\textbf{Simulation Setup}}\\
\hline
% Final Time $t_{f}$, s & 120 & Time Step $\Delta$t, s & 10$^{-3}$\\
Time Step $\Delta$t, s & 10$^{-2}$\\
\hline
\label{tab:nominalparams}\\
\end{tabular}
